On reduced modeling of the modulational dynamics in magnetohydrodynamics

This paper explores structure formation in two-dimensional magnetohydrodynamic (MHD) turbulence as a modulational instability (MI) of turbulent fluctuations. We focus on the early stages of structure formation and consider simple backgrounds that allow for a tractable model of the MI while retaining the full chain of modulational harmonics. This approach allows us to systematically examine the validity of popular closures such as the quasilinear approximation and other low-order truncations. We find that, although such simple closures can provide quantitatively accurate approximations of the MI growth rates in some regimes, they can fail to capture the modulational dynamics in adjacent regimes even qualitatively, falsely predicting MI when the system is actually stable. We find that this discrepancy is due to the excitation of propagating spectral waves (PSWs) which can ballistically transport energy along the modulational spectrum, unimpeded until dissipative scales, thereby breaking the feedback loops that would otherwise sustain MIs. PSWs can be self-maintained as global modes with real frequencies and drain energy from the primary structure at a constant rate until the primary structure is depleted. To describe these waves within a reduced model, we propose an approximate spectral closure that captures them and MIs on the same footing. We also find that introducing corrections to ideal MHD, conservative or dissipative, can suppress PSWs and reinstate the accuracy of the quasilinear approximation. In this sense, ideal MHD is a `singular' system that is particularly sensitive to the accuracy of the closure within mean-field models.

==> old.tex <==
\sjnew{
Although all closures, in any context, ultimately rely on a truncation of a formally infinite chain of correlations\footnote{Here, we use the term `truncation' to refer to low-order closures in general, as opposed to precisely the closure choice of setting all correlations to zero  after some cutoff. The latter, which we will refer to as a simple truncation, is done in the quasilinear approximation but not, for example, in the various \m{\tau} approximations \citep{ref:brandenburg05, ref:blackman02}.}, the matter calls for special attention in this case. In typical closure problems, the fluctuations are small compared to the mean field. In turbulent structure formation, though, the usual roles of perturbation and background are switched. A turbulent field per~se typically has a zero average, while second- and higher-order functionals of it are not, and they serve as a background on top of which the coherent mean field resides as a perturbation. Here, the question of closure validity is therefore particularly delicate.

Consider, as a representative and popular example, the so-called first-order smoothing \citep{book:krause80}, or second-order correlation approximation \citep{ref:radler82}, which implies that the mean-field evolution is determined only by second-order correlations of the fluctuations. This approximation is also called quasilinear, and, fundamentally, the resulting models are concerned with quasilinear ponderomotive effects \citep{my:ql}. 

On the one hand, the regime of validity is, formally, extremely limited. Based on a ordering of terms in the induction equation, it can be rigorously justified only for small magnetic Reynolds numbers or short correlation times \citep{ref:brandenburg05_rev, ref:rincon19}. Comparisons with direct numerical simulations often corroborate this \citep{ref:pipin08, ref:schrinner05}. On the other hand, it endures in its popularity as a workhorse that is too convenient to cast aside in analytical calculations \citep{ref:squire15_a, ref:lingam16, ref:masada14, ref:gopalakrishnan23}. Furthermore, quasilinear calculations have sometimes been found to produce surprisingly good agreement with direct numerical simulations (DNS) outside of the formal regime of validity \citep{ref:kapyla06}. \footnote{Adding to the complication, the various analytical closures and DNS can conflict and agree in various combinations \citep{ref:zhou21}.} It is therefore worth seeking a higher resolution understanding of the validity of these simple closures; when, and why exactly, do they fail? Answering this question requires exploring a fully non-truncated mean-field model.}
